An Integrated Mechanical Intelligence and Control Approach Towards Flight Control of Aerobat

Our goal in this work is to expand the theory and practice of robot locomotion by addressing critical challenges associated with the robotic biomimicry of bat aerial locomotion. Bats are known for their pronounced, fast wing articulations, e.g., bats can mobilize as many as forty joints during a single wingbeat, with some joints reaching over one thousand degrees per second in angular speed. Copying bats flight is a significant ordeal, however, very rewarding. Aerial drones with morphing bodies similar to bats can be safer, agile and energy-efficient owing to their articulated and soft wings. Current design paradigms have failed to copy bat flight because they assume only closed-loop feedback roles and ignore computational roles carried out by morphology. To respond to the urgency, a design framework called Morphing via Integrated Mechanical Intelligence and Control (MIMIC) is proposed. In this paper, using the dynamic model of Northeastern University's Aerobat, which is designed to test the effectiveness of the MIMIC framework, it will be shown that computational structures and closed-loop feedback can be successfully used to mimic bats stable flight apparatus.

==> old_content.tex <==
\begin{comment}

 The links dimensions are constant except for the 
 
 
 The body frame positions of the massless linkages are defined using the following relations

{\color{red} Redundant Eqs.!}
%
\begin{equation}
\begin{aligned}
    \bm p_{3A}^B &= \bm p_4^B + R(\theta_4)\bm l_3, \\
    \bm p_{11A}^B &= \bm p_{12}^B + R(\theta_{12})\bm l_{8a} \\
    \bm p_{15A}^B &= \bm p_{14}^B + R(\theta_{14})\bm l_{10}, \\
    \bm p_{3B}^B &= \bm p_1^B + R(\theta_1)\bm l_1 + R(\theta_2)\bm l_2 \\
    \bm p_{11B}^B &= \bm p_{9}^B + R(\theta_9)\bm l_6 + R(\theta_{10})\bm l_7 \\
    \bm p_{15B}^B &= \bm p_{12}^B + R(\theta_{12})\bm l_{8b} + R(\theta_{13})\bm l_9
\end{aligned}
\label{eq:kinematics}
\end{equation}
%
where $\bm p_{iA}$ and $\bm p_{iA}$ for $i=\{3, 11, 15\}$ are the position of the $i$'th joint found from two different sides in the chain. $\bm p_{i}^B$ for $i = \{ 1, 4, 9, 12, 14 \}$ is the position of the corresponding fixed joints in the body frame, which can be found in Table \ref{tab:param_values}. $R(\cdot)$ is the rotation matrix from  link frame to the body frame, which is a function of link's absolute angle $\theta_i$ about the body frame. $\bm l_i$ for $i = \{ 2, 3, 7, 8, 9, 10 \}$ is the $i$th joints' position defined in its corresponding link frame which could be either fixed or variable depending on the link. For the links attached to the prismatic joints shown in Fig. \ref{fig:wing_structure_dimensions}, we have $\bm l_3 = [-l_{3b}-l_{3c},0]^\top$, $\bm l_{8a} = [-l_{8a}-l_{8b},0]^\top$, $\bm l_{8b}=[-l_{8b},l_{8c}]^\top$, $\bm l_{9} = [l_9,0]^\top$, and $\bm l_{10} = [-l_{10a},l_{10b}]^\top$. 

Let $\bm{q}_1$ be the vector of generalized coordinates for the massless system consisting of the 12 states for one side of the wing, where
\begin{equation}
\bm q_1 =[\theta_1,\theta_2, \theta_4,\theta_9,\theta_{10},\theta_{12}, \theta_{13},\theta_{14}, l_{3b}, l_{3c},\\ l_{8b}, l_{10b}]^\top.    
\label{eq:states_massless}
\end{equation}
%


\begin{table}[t]
\centering
\caption{Wing Specifications}
\begin{tabular}{cc|cc|cc}
%\hline 
Param. & Value & Param. & Value & Param. & Value \\
\hline$l_{1}$ & $3.88 \mathrm{mm}$ & $l_{8 c}$ & $10.0 \mathrm{mm}$ & $p_{4 x}^{*}$ & $=l_{3 a}$ \\
$l_{2}$ & $11.5 \mathrm{mm}$ & $l_{9}$ & $9.01 \mathrm{mm}$ & $p_{4 y}$ & $2.90 \mathrm{mm}$ \\
$l_{3 a}$ & $14.7 \mathrm{mm}$ & $l_{10 a}$ & $5.00 \mathrm{mm}$ & $p_{7 x}$ & $17.5 \mathrm{mm}$ \\
$l_{3 b}$ & $6.91 \mathrm{mm}$ & $l_{10 b}$ & $7.00 \mathrm{mm}$ & $p_{7 y}$ & $10.4 \mathrm{mm}$ \\
$l_{3 c}$ & $11.0 \mathrm{mm}$ & $l_{10 c}$ & $70.0 \mathrm{mm}$ & $p_{9 y}^{*}$ & $-15 \mathrm{mm}$ \\
$l_{4}$ & $9.46 \mathrm{mm}$ & $l_{10 d}$ & $9.40 \mathrm{mm}$ & $p_{12 x}^{*}$ & $=l_{8 a}$ \\
$l_{5 a}$ & $3.35 \mathrm{mm}$ & $l_{11}$ & $25.1 \mathrm{mm}$ & $p_{12 y}$ & $-5.00 \mathrm{mm}$ \\
$l_{5 b}$ & $4.56 \mathrm{mm}$ & $l_{12 a}$ & $30.0 \mathrm{mm}$ & $p_{14 x}$ & $15.8 \mathrm{mm}$ \\
$l_{6}$ & $3.46 \mathrm{mm}$ & $l_{12 b}$ & $9.98 \mathrm{mm}$ & $p_{14 y}$ & $4.68 \mathrm{mm}$ \\
$l_{7}$ & $12.0 \mathrm{mm}$ & $l_{h}^{*}$ & $50 \mathrm{mm}$ & $\alpha_{5}$ & $31.0^{\circ}$ \\
$l_{8 a}$ & $10.0 \mathrm{mm}$ & $l_{r}^{*}$ & $90 \mathrm{mm}$ & $\phi_{0}$ & $1^{\circ}$ \\
$l_{8 b}$ & $7.00 \mathrm{mm}$ & $p_{1 y}^{*}$ & $15 \mathrm{mm}$ & $\Delta \phi$ & $18.2^{\circ}$ \\
\hline
\end{tabular}
\label{tab:param_values}
\end{table}
%

\begin{equation}
    \begin{aligned}
\bm \Pi_B &= R_B I_B \bm \omega_B - m_B\left(\bm x_B -\bm x_{CoM}\right) \times \bm v_B \\
\bm \Pi_{LH} &= R_B I_H \bm \omega_{LH} - m_H\left(\bm x_{LH} -\bm x_{CoM}\right) \times \bm v_{LH} \\
\bm \Pi_{LR} &= R_B I_R \bm \omega_{LR} - m_R\left(\bm x_{LR} -\bm x_{CoM}\right) \times \bm v_{LR} \\
   \end{aligned}
\end{equation}


\begin{equation}
    \begin{bmatrix}
       M_1& 0_{12 \times 10}\\
       0_{10 \times 12}& M_2
    \end{bmatrix} \, 
    \ddot{\bm{q}} + 
    \begin{bmatrix}
       \bm{h}_1 \\ \bm{h}_2
    \end{bmatrix} = 
    \begin{bmatrix}
        B_1 \bm u_1 \\
        \bm u_2
    \end{bmatrix}  
\label{eq:eom_full}    
\end{equation}
%
where $\ddot \bm{q} = [\\bm{q}_1^\top, \bm{q}_2^{\top}, \bm{\omega}]^\top$. Finally, the Additionally, we update the rotation matrix $R_B$ using the $\dot R_B$ in \eqref{eq:eom_bodyrot}.

The $B_i$ matrix is derived as follows
\begin{equation}
    B_i = \\\frac {\partial {}} {\partial{\dot {\bm q}_2}}
    \begin{bmatrix}
    \delta \bm \omega_{LH}&
    \delta \bm \omega_{LR}&
    \delta \bm \omega_{RH}&
    \delta \bm \omega_{RR}
    \end{bmatrix}^\top
\end{equation}
where $\dot {\bm q}_2 =[\dot \theta_{Ls}, \dot \theta_{Le}, \dot \theta_{Rs}, \dot \theta_{Re}, \bm {\dot x}_B, \bm \omega_B]^\top $ and $\delta \bm \omega_i = \bm \omega_i - \bm \omega_B$.



{\color{red} Redundant Eqs.!}

%
\begin{equation}
\begin{aligned}
    &\bm u_g(\bm q_1, \bm q_2)=\\&k_{g}
    \begin{bmatrix}
     |\bm p_{L5}- \bm p_{L6}|-l_4 \\
     |\bm p_{L16}-\bm p_{L16}|-l_{11}  \\
     |\bm p_{R5}- \bm p_{R6}|-l_4  \\
     |\bm p_{R16}-\bm p_{R16}|-l_{11}\\
    \end{bmatrix}
    \begin{bmatrix}
    \bm e_{L6}\\
    \bm e_{L17}\\
    \bm e_{R6}\\
    \bm e_{R17}
    \end{bmatrix}\\+ &b_{g} 
    \begin{bmatrix}
    (\bm {\dot p}_{L5} -\bm {\dot p}_{L6})^\top \bm e_{L6}\\
    (\bm {\dot p}_{L16}- \bm {\dot p}_{L17})^\top \bm e_{L17}\\
    (\bm {\dot p}_{R5} - \bm {\dot p}_{R6})^\top \bm e_{R6}\\ 
    (\bm {\dot p}_{R16}- \bm {\dot p}_{R17})^\top \bm e_{R17} 
    \end{bmatrix}
    \begin{bmatrix}
    \bm e_{L6}\\
    \bm e_{L17}\\
    \bm e_{R6}\\
    \bm e_{R17}
    \end{bmatrix}
\end{aligned}
\end{equation}

where $\bm e_{6} = \frac {\bm p_{5}-\bm p_{6}}{|\bm p_{5}-\bm p_{6}|}$ and $\bm e_{17}= \frac {\bm p_{16}-\bm p_{17}}{|\bm p_{16}-\bm p_{17}|}$ hold for both wings. $k_{g}$ and $b_g$ are the linear spring stiffness and damping coefficient, respectively. Additionally, $\bm p_{Li}$ for $i=\{5, 6, 16, 17$\} is the inertial position of the corresponding joints in the left wing which can be calculated by the following equations.

{\color{red} Redundant Eqs.!}

\begin{equation}
    \begin{aligned}
    \bm p_{L5} &= \bm p_{L4} + R(\theta_4)\bm [0,-l_{3b},l_{3c}]^\top\\
    \bm p_{L6} &= \bm p_{L7} +  R(\theta_7) [0,-l_{5a},l_{5b}]^\top\\
    \bm p_{L16} &= \bm p_{L14} + R(\theta_{14})[0,l_{10c},l_{10d}+l_{10b}-l_{10b}(0)]^\top\\
    \bm p_{L17} &= \bm p_{L7} + R(\theta_7)[0,l_{5c}\cos(\alpha),l_{5b}+l_{5c}\sin(\alpha)]^\top+\\
    &R(\theta_8)[0,l_{12a},l_{12b}]^\top\\
    \end{aligned}
\end{equation}
 $\bm p_{L4}$, $\bm p_{L7}$, and $\bm p_{L14}$ are the position of the fixed joints attached to the body. The same positions for the right wing can be found using above equations with considerations on $y$-axis components. The corresponding coefficient matrix is as below. 
 \begin{equation}
    B_g = \frac {\partial{}}{\partial {\dot{\bm q}_2}}
    \begin{bmatrix}
    {\delta \bm {\dot p}_{L6}}&
    {\delta \bm {\dot p}_{L17}}&
    {\delta \bm {\dot p}_{R6}}&
    {\delta \bm {\dot p}_{R17}}
    \end{bmatrix}^\top
\end{equation}
in which $\delta \bm {\dot p}_{Li}=\bm {\dot p}_{Li-1}- \bm {\dot p}_{Li}$  for $i=\{6, 17\}$.


\end{comment}
